HPDR: High-Performance Portable Scientific Data Reduction Framework

The rapid growth of scientific data is surpassing advancements in computing, creating challenges in storage, transfer, and analysis, particularly at the exascale. While data reduction techniques such as lossless and lossy compression help mitigate these issues, their computational overhead introduces new bottlenecks. GPU-accelerated approaches improve performance but face challenges in portability, memory transfer, and scalability on multi-GPU systems. To address these, we propose HPDR, a high-performance, portable data reduction framework. HPDR supports diverse processor architectures, reducing memory transfer overhead to 2.3% and achieving up to 3.5x faster throughput than existing solutions. It attains 96% of the theoretical speedup in multi-GPU settings. Evaluations on the Frontier supercomputer demonstrate 103 TB/s throughput and up to 4x acceleration in parallel I/O performance at scale. HPDR offers a scalable, efficient solution for managing massive data volumes in exascale computing environments.

==> tex/related_works.tex <==
\section{Related Works}
%SZ-HDF5 work, WRF-ADIOS lossless work, etc.
\subsection{ADIOS with Lossless compressor}
The Weather Research and Forecasting Model (WRF) [] represents a cutting-edge numerical weather prediction system developed for both weather forecasting and atmospheric research. WRF generates a substantial number of variables when stimulating multiple physics processes.  
In a study [], researchers investigated the impact of in-line lossless compressors on write times with WRF code. They employed ADIOS2 as the I/O backend for writing and compressing data at each time step. The study evaluated 4 lossless compressors implemented on CPU – BloscLZ [], LZ4 [], Zlib [], Zstandard [] -- integrated within ADIOS data management library. The experimental results show that utilizing ADIOS2 with lossless compression on CPUs led to approximately 50\% reduction in average write time compared to uncompressed configurations, accompanied by a $4\times$ reduction in output size. 
\subsection{HDF5 with lossy compressor}
Recently efforts have explored the use of lossy compression to accelerate I/O, as it can significantly reduce data volume while ensuring that the reduced quality meets application requirements. In [], authors integrated a predictive lossy compressor with the HDF5 parallel I/O library. Conventionally, parallel writing of a dataset requires data to be partitioned into chunks of equal size for simultaneous processing by different processors. In contrast to our end-to-end optimization approach, the work in [] focused on addressing the unbalanced I/O times caused by the varied data size after compression across different partitions. It used learned information to enable asynchronous writing with lossy compression across consecutive time steps. However, this approach primarily considered a CPU-based compressor and evaluated the throughput improvement against I/O times obtained in a nonideal setting. For instance, the paper compared the combined time spent on compression and writing reduced data against the time taken for writing uncompressed data using HDF5, with the latter delivering an I/O throughput of approximately 750MB/sec per processor. In comparison, our experiments leverage the state-of-the-art parallel I/O library ADIOS2, which boasts a peak I/O throughput of XX. Our findings underscore two key insights: (1) With a meticulously optimized GPU compressor, the bottleneck shifts to CPU-GPU data movement, highlighting the need for enhancing the overlap efficiency between compression and inter-device data transfer. (2) When I/O operations achieve sufficient speed, compression can expediate I/O solely through GPU utilization and comprehensive end-to-end pipeline optimization.  

